MM-Embed: Universal Multimodal Retrieval with Multimodal LLMs

State-of-the-art retrieval models typically address a straightforward search scenario, in which retrieval tasks are fixed (e.g., finding a passage to answer a specific question) and only a single modality is supported for both queries and retrieved results. This paper introduces techniques for advancing information retrieval with multimodal large language models (MLLMs), enabling a broader search scenario, termed universal multimodal retrieval, where multiple modalities and diverse retrieval tasks are accommodated. To this end, we first study fine-tuning an MLLM as a bi-encoder retriever on 10 datasets with 16 retrieval tasks. Our empirical results show that the fine-tuned MLLM retriever is capable of understanding challenging queries, composed of both text and image, but it underperforms compared to a smaller CLIP retriever in cross-modal retrieval tasks due to the modality bias exhibited by MLLMs. To address the issue, we propose modality-aware hard negative mining to mitigate the modality bias exhibited by MLLM retrievers. Second, we propose continuously fine-tuning the universal multimodal retriever to enhance its text retrieval capability while preserving multimodal retrieval capability. As a result, our model, MM-Embed, achieves state-of-the-art performance on the multimodal retrieval benchmark M-BEIR, which spans multiple domains and tasks, while also surpassing the state-of-the-art text retrieval model, NV-Embed-v1, on the MTEB retrieval benchmark. We also explore prompting the off-the-shelf MLLMs as zero-shot rerankers to refine the ranking of the candidates from the multimodal retriever. We find that, through prompt-and-reranking, MLLMs can further improve multimodal retrieval when the user queries (e.g., text-image composed queries) are more complex and challenging to understand. These findings also pave the way for advancing universal multimodal retrieval in the future.

==> circo_experiments.tex <==
% \begin{table}[h]
\begin{wraptable}{r}{0.3\columnwidth}
% \vspace{-4mm}
	\caption{\footnotesize
 Experiment on composed image retrieval task, CIRCO~\citep{circo}.}
	\label{tb:circo_result}
	\centering
	 \resizebox{0.3\columnwidth}{!}{  
	  \setlength\tabcolsep{0.1cm}
    \begin{tabular}{l|cc}
\hline \hline
Model& Ret.& Rerank\\
 \hline
 MagicLens& 24.9& 32.4 \\
E5-V& 19.1& 31.0\\
% CLIP + NVEmb (no training)& -& 25.8\\
$M^{\text{rand}}$(\clipsf{})& 12.7& 31.6 \\
% \blipff~\citep{uniir}& 26.6& 36.1 \\
% \llavanext& 28.3& 37.0\\
% \nvembed& 29.3& 36.6\\
$M^{\text{hard}}$ (\promptllavanext)& 29.0& 37.9\\
$M^{\text{hard}}$ (\nvembed)& 32.4& 40.9\\
\ourmodel& 32.3& 39.9 \\
\hline \hline
	\end{tabular}
	}
 \vspace{-0.4cm}
\end{wraptable}
% \end{table}
